PromptRR: Diffusion Models as Prompt Generators for Single Image Reflection Removal

Existing single image reflection removal (SIRR) methods using deep learning tend to miss key low-frequency (LF) and high-frequency (HF) differences in images, affecting their effectiveness in removing reflections. To address this problem, this paper proposes a novel prompt-guided reflection removal (PromptRR) framework that uses frequency information as new visual prompts for better reflection performance. Specifically, the proposed framework decouples the reflection removal process into the prompt generation and subsequent prompt-guided restoration. For the prompt generation, we first propose a prompt pre-training strategy to train a frequency prompt encoder that encodes the ground-truth image into LF and HF prompts. Then, we adopt diffusion models (DMs) as prompt generators to generate the LF and HF prompts estimated by the pre-trained frequency prompt encoder. For the prompt-guided restoration, we integrate specially generated prompts into the PromptFormer network, employing a novel Transformer-based prompt block to effectively steer the model toward enhanced reflection removal. The results on commonly used benchmarks show that our method outperforms state-of-the-art approaches. The codes and models are available at https://github.com/TaoWangzj/PromptRR.

==> images_latex/figure_result2.tex <==
\def \rootpostcardv2 {images_supp/datasets-v2/postcard/origin_img_with_box/}
\begin{figure*}[ht]
    \centering
    \resizebox{0.88\textwidth}{!}{
    \begin{minipage}{\textwidth}
      \centering
    \begin{subfigure}[t]{0.24\linewidth}
        \includegraphics[width=\linewidth]{\rootpostcardv2 input/input_ea-5-m-11.pdf}
        \caption{\small Input (PSNR: 21.23)}
    \end{subfigure}
    \hspace{-5pt}
    \begin{subfigure}[t]{0.24\linewidth}
        \includegraphics[width=\linewidth]{\rootpostcardv2 WY19/WY19_ea-5-m-11.pdf}
        \caption{\small WY19 (PSNR: 20.16)}
    \end{subfigure}
    \hspace{-5pt}
    \begin{subfigure}[t]{0.24\linewidth}
        \includegraphics[width=\linewidth]{\rootpostcardv2 WT19/WT19_ea-5-m-11.pdf}
        \caption{\small WT19 (PSNR: 7.17)}
    \end{subfigure}
    \hspace{-5pt}
    \begin{subfigure}[t]{0.24\linewidth}
        \includegraphics[width=\linewidth]{\rootpostcardv2 LY20/LY20_ea-5-m-11.pdf}
        \caption{\small LY20 (PSNR: 17.42)}
    \end{subfigure}
    \\ % New row
    \begin{subfigure}[t]{0.24\linewidth}
        \includegraphics[width=\linewidth]{\rootpostcardv2 ZS21/ZS21_ea-5-m-11.pdf}
        \caption{\small ZS21 (PSNR: 16.10)}
    \end{subfigure}
    \hspace{-5pt}
    \begin{subfigure}[t]{0.24\linewidth}
        \includegraphics[width=\linewidth]{\rootpostcardv2 CL21/CL21_ea-5-m-11.pdf}
        \caption{\small CL21 (PSNR: 19.34)}
    \end{subfigure}
    \hspace{-5pt}
    \begin{subfigure}[t]{0.24\linewidth}
        \includegraphics[width=\linewidth]{\rootpostcardv2 HG21/HG21_ea-5-m-11.pdf}
        \caption{\small HG21 (PSNR: 21.11)}
    \end{subfigure}
    \hspace{-5pt}
    \begin{subfigure}[t]{0.24\linewidth}
        \includegraphics[width=\linewidth]{\rootpostcardv2 Uformer/Uformer_ea-5-m-11.pdf}
        \caption{\small Uformer (PSNR: 16.95)}
    \end{subfigure}
    \\ % New row
    \begin{subfigure}[t]{0.24\linewidth}
        \includegraphics[width=\linewidth]{\rootpostcardv2 Restormer/Restormer_ea-5-m-11.pdf}
        \caption{\small Restormer (PSNR: 11.05)}
    \end{subfigure}
    \hspace{-5pt}
    \begin{subfigure}[t]{0.24\linewidth}
        \includegraphics[width=\linewidth]{\rootpostcardv2 RSIRR/RSIRR_ea-5-m-11.pdf}
        \caption{\small RSIRR (PSNR: 19.06)}
    \end{subfigure}
    \hspace{-5pt}
    \begin{subfigure}[t]{0.24\linewidth}
        \includegraphics[width=\linewidth]{\rootpostcardv2 PromptRR/PromptRR_ea-5-m-11.pdf}
        \caption{\small Ours (PSNR: 28.19)}
    \end{subfigure}
    \hspace{-5pt}
    \begin{subfigure}[t]{0.24\linewidth}
        \includegraphics[width=\linewidth]{\rootpostcardv2 GT/GT_ea-5-m-11.pdf}
        \caption{\small GT}
    \end{subfigure}
    \end{minipage}
}
    \caption{Visual comparison on \textit{PostCard}~\cite{Wan_2017_iccv} dataset. \textbf{Zoom-in for better details}.}
    \label{results_fig3}
     \vspace{-5mm}
\end{figure*}

==> images_latex/figure_result3.tex <==
\def \rootsolidobjectv2 {images_supp/datasets-v2/solidobject/origin_img_with_box/}

\begin{figure*}[h]
    \centering
        \resizebox{0.88\textwidth}{!}{
    \begin{minipage}{\textwidth}
      \centering
    \begin{subfigure}[t]{0.24\linewidth}
        \includegraphics[width=\linewidth]{\rootsolidobjectv2 input/input_14-Focus-11-m.pdf}
        \caption{\small Input (PSNR: 22.56)}
    \end{subfigure} \hspace{-5pt}
    \begin{subfigure}[t]{0.24\linewidth}
        \includegraphics[width=\linewidth]{\rootsolidobjectv2 WY19/WY19_14-Focus-11-m.pdf}
        \caption{\small WY19 (PSNR: 22.23)}
    \end{subfigure} \hspace{-5pt}
    \begin{subfigure}[t]{0.24\linewidth}
        \includegraphics[width=\linewidth]{\rootsolidobjectv2 WT19/WT19_14-Focus-11-m.pdf}
        \caption{\small WT19 (PSNR: 10.10)}
    \end{subfigure} \hspace{-5pt}
    \begin{subfigure}[t]{0.24\linewidth}
        \includegraphics[width=\linewidth]{\rootsolidobjectv2 LY20/LY20_14-Focus-11-m.pdf}
        \caption{\small LY20 (PSNR: 23.36)}
    \end{subfigure} 
    \\  % Newline for better spacing
    \begin{subfigure}[t]{0.24\linewidth}
        \includegraphics[width=\linewidth]{\rootsolidobjectv2 ZS21/ZS21_14-Focus-11-m.pdf}
        \caption{\small ZS21 (PSNR: 18.51)}
    \end{subfigure} \hspace{-5pt}
    \begin{subfigure}[t]{0.24\linewidth}
        \includegraphics[width=\linewidth]{\rootsolidobjectv2 CL21/CL21_14-Focus-11-m.pdf}
        \caption{\small CL21 (PSNR: 23.92)}
    \end{subfigure} \hspace{-5pt}
    \begin{subfigure}[t]{0.24\linewidth}
        \includegraphics[width=\linewidth]{\rootsolidobjectv2 HG21/HG21_14-Focus-11-m.pdf}
        \caption{\small HG21 (PSNR: 21.84)}
    \end{subfigure} \hspace{-5pt}
    \begin{subfigure}[t]{0.24\linewidth}
        \includegraphics[width=\linewidth]{\rootsolidobjectv2 Uformer/Uformer_14-Focus-11-m.pdf}
        \caption{\small Uformer (PSNR: 22.63)}
    \end{subfigure} 
    \\  % Newline for better spacing
    \begin{subfigure}[t]{0.24\linewidth}
        \includegraphics[width=\linewidth]{\rootsolidobjectv2 Restormer/Restormer_14-Focus-11-m.pdf}
        \caption{\small Restormer (PSNR: 25.23)}
    \end{subfigure} \hspace{-5pt}
    \begin{subfigure}[t]{0.24\linewidth}
        \includegraphics[width=\linewidth]{\rootsolidobjectv2 RSIRR/RSIRR_14-Focus-11-m.pdf}
        \caption{\small RSIRR (PSNR: 24.98)}
    \end{subfigure} \hspace{-5pt}
    \begin{subfigure}[t]{0.24\linewidth}
        \includegraphics[width=\linewidth]{\rootsolidobjectv2 PromptRR/PromptRR_14-Focus-11-m.pdf}
        \caption{\small Ours (PSNR: 25.84)}
    \end{subfigure} \hspace{-5pt}
    \begin{subfigure}[t]{0.24\linewidth}
        \includegraphics[width=\linewidth]{\rootsolidobjectv2 GT/GT_14-Focus-11-m.pdf}
        \caption{\small GT}
    \end{subfigure}   
   \end{minipage}
}
    \caption{Visual comparison on \textit{SolidObject}~\cite{Wan_2017_iccv} dataset. \textbf{Zoom-in for better details}.}
    \label{results_fig6}
    \vspace{-5mm}
\end{figure*}

==> images_latex/figure_result4.tex <==

\def \rootwildv2 {images_supp/datasets-v2/wild_v2/}

\begin{figure*}[h]
    \centering
    \resizebox{0.88\textwidth}{!}{  % Scale the figure, adjust as needed
    \begin{minipage}{\textwidth}
        \centering
        \begin{subfigure}{0.24\linewidth}
            \includegraphics[width=\linewidth]{\rootwildv2 input_22s-m.pdf}
            \caption{\small Input (PSNR: 14.80)}
        \end{subfigure} \hspace{-3pt}
        \begin{subfigure}{0.24\linewidth}
            \includegraphics[width=\linewidth]{\rootwildv2 WY19_22s-m.pdf}
            \caption{\small WY19 (PSNR: 21.31)}
        \end{subfigure} \hspace{-3pt}
        \begin{subfigure}{0.24\linewidth}
            \includegraphics[width=\linewidth]{\rootwildv2 WT19_22s-m.pdf}
            \caption{\small WT19 (PSNR: 12.99)}
        \end{subfigure} \hspace{-3pt}
        \begin{subfigure}{0.24\linewidth}
            \includegraphics[width=\linewidth]{\rootwildv2 LY20_22s-m.pdf}
            \caption{\small LY20 (PSNR: 23.78)}
        \end{subfigure} 
        \\  % New row
        \begin{subfigure}{0.24\linewidth}
            \includegraphics[width=\linewidth]{\rootwildv2 ZS21_22s-m.pdf}
            \caption{\small ZS21 (PSNR: 22.91)}
        \end{subfigure} 
        \begin{subfigure}{0.24\linewidth}
            \includegraphics[width=\linewidth]{\rootwildv2 CL21_22s-m.pdf}
            \caption{\small CL21 (PSNR: 19.88)}
        \end{subfigure} \hspace{-3pt}
        \begin{subfigure}{0.24\linewidth}
            \includegraphics[width=\linewidth]{\rootwildv2 HG21_22s-m.pdf}
            \caption{\small HG21 (PSNR: 17.14)}
        \end{subfigure} \hspace{-3pt}
        \begin{subfigure}{0.24\linewidth}
            \includegraphics[width=\linewidth]{\rootwildv2 Uformer_22s-m.pdf}
            \caption{\small Uformer (PSNR: 18.17)}
        \end{subfigure} 
        \\  % New row
        \begin{subfigure}{0.24\linewidth}
            \includegraphics[width=\linewidth]{\rootwildv2 Restormer_22s-m.pdf}
            \caption{\small Restormer (PSNR: 29.55)}
        \end{subfigure} \hspace{-3pt}
        \begin{subfigure}{0.24\linewidth}
            \includegraphics[width=\linewidth]{\rootwildv2 RSIRR_22s-m.pdf}
            \caption{\small RSIRR (PSNR: 16.99)}
        \end{subfigure}
        \begin{subfigure}{0.24\linewidth}
            \includegraphics[width=\linewidth]{\rootwildv2 PromptRR_22s-m.pdf}
            \caption{\small Ours (PSNR: 31.07)}
        \end{subfigure} \hspace{-3pt}
        \begin{subfigure}{0.24\linewidth}
            \includegraphics[width=\linewidth]{\rootwildv2 GT_22s-m.pdf}
            \caption{\small GT}
        \end{subfigure}  
    \end{minipage}
    }  % End of resizebox
    
    \caption{Visual comparison on \textit{WildScene}~\cite{Wan_2017_iccv} dataset. \textbf{Zoom-in for better details}.}
    \label{results_fig7}
    % \vspace{-5mm}  % Adjust vertical space after figure
\end{figure*}

==> images_latex/results_natures.tex <==

\begin{figure*}[t]
 \begin{center}
   \begin{overpic}[width=0.95\textwidth]{images/nature_comparison.pdf}
     \put(5,-1.5){Input}
   \put(16.5,-1.5){CL21}
   \put(28.5,-1.5){HG21}
   \put(40,-1.5){Uformer}
   \put(52.5,-1.5){Restormer}
   \put(66,-1.5){RSIRR}
   \put(77,-1.5){PromptRR}
   \put(91.5,-1.5){GT}
  \end{overpic}
  \vspace{8pt}
	% \caption{Visual comparison on \textit{Nature} dataset. Compared with other methods, our PromptRR effectively removes reflections while preserving the fine details in the restored images.}
 	\caption{Visual comparison on \textit{Nature} dataset.}
 	\label{fig:results_nature}
 	\end{center}
    % \vspace{-4mm}
 \end{figure*}

==> images_latex/results_real20.tex <==
\begin{figure*}[t]
 \begin{center}
   \begin{overpic}[width=\textwidth]{images/real_comparison.pdf}
     \put(5,-1.5){Input}
   \put(16.5,-1.5){CL21}
   \put(28.5,-1.5){HG21}
   \put(40,-1.5){Uformer}
   \put(52.5,-1.5){Restormer}
   \put(66,-1.5){RSIRR}
   \put(77,-1.5){PromptRR}
   \put(91.5,-1.5){GT}
  \end{overpic}
  \vspace{6pt}
	% \caption{Visual comparison on \textit{Real} dataset. The reflection results of comparison methods still contain significant reflection effects. Our PromptRR removes the reflection areas more accurately and thoroughly.}
 	\caption{Visual comparison on \textit{Real} dataset.}
 	\label{fig:results_real}
 	\end{center}
  % \vspace{-3mm}
 \end{figure*}

==> table_latex/efficiency_analysis.tex <==
\begin{table}[t] \small
	\centering
	\caption{Efficiency comparison of recent SOTA methods.}
	% \vspace{-3mm}
	\resizebox{0.9\columnwidth}{!}{
	\begin{tabular}{ccccc}
	\hline 
	Methods        &  Restormer   & Uformer & RSIRR &   PromptRR                  \\ \hline
	Speed  &  &  &  &  \\ 
        Parameter  &  &  &  &  \\ 
        GFlops  &  &  &  &  \\ \hline 
\end{tabular}
	}	
	\label{table_efficiency_comparison}
	% \vspace{-4mm}
\end{table}



